Categorical Tools for Natural Language Processing

This thesis develops the translation between category theory and computational linguistics as a foundation for natural language processing. The three chapters deal with syntax, semantics and pragmatics. First, string diagrams provide a unified model of syntactic structures in formal grammars. Second, functors compute semantics by turning diagrams into logical, tensor, neural or quantum computation. Third, the resulting functorial models can be composed to form games where equilibria are the solutions of language processing tasks. This framework is implemented as part of DisCoPy, the Python library for computing with string diagrams. We describe the correspondence between categorical, linguistic and computational structures, and demonstrate their applications in compositional natural language processing.

==> 0.2-publications.tex <==


The material presented in this thesis builds on the following publications.

\begin{itemize}
    \item \enumcite{coecke2018c}
    \item \enumcite{defelice2020}
    \item \enumcite{defelice2020b}
    \item \enumcite{meichanetzidis2020}
    \item \enumcite{meichanetzidis2020a}
    \item \enumcite{coecke2020a}
    \item \enumcite{defelice2020a}
\end{itemize}

During his DPhil, the author has also published the following articles.

\begin{itemize}
    \item \enumcite{defelice2019}
    \item \enumcite{backens2020}
    \item \enumcite{toumi2021a}
    \item \enumcite{kartsaklis2021}
    \item \enumcite{coecke2022}
    \item \enumcite{dilavore2022}
    \item \enumcite{defelice2022}
    \item \enumcite{toumi2022}
\end{itemize}


==> 2.a-tensornetwork.tex <==


We describe the implementation of the class
\py{tensor.Diagram} which can be used as a middle step for evaluating any DisCoPy
\py{Diagram} as a tensor network. It forms in fact an implementation of tensor networks
with a specified contraction order given by the premonoidal structure of \py{Diagram}.
We describe the interface between \py{tensor.Diagram} and Google's library
\py{tensornetwork}.

A \py{tensor.Diagram} is a diagram in a premonoidal category with special
morphisms \py{cups}, \py{caps} making it a rigid category, as well as \py{spiders}
and \py{swap} for the hypergraph structure. We implement it as a subclass of
\py{rigid.Diagram}.

\begin{python}\label{listing:tensor.Diagram}
{\normalfont Diagrams with Tensor boxes}

\begin{minted}{python}
@monoidal.Diagram.subclass
class Diagram(rigid.Diagram):

    @staticmethod
    def cups(left, right):
        return rigid.cups(left, right, ar_factory=Diagram,
                          cup_factory=lambda x, _: Spider(2, 0, x[0]))

    @staticmethod
    def caps(left, right):
        return Diagram.cups(left, right).dagger()

    @staticmethod
    def swap(left, right):
        return monoidal.Diagram.swap(
            left, right, ar_factory=Diagram, swap_factory=Swap)

    @staticmethod
    def spiders(n_legs_in, n_legs_out, dim):
        dim = dim if isinstance(dim, Dim) else Dim(dim)
        if not dim:
            return Id(dim)
        if len(dim) == 1:
            return Spider(n_legs_in, n_legs_out, dim)
        raise NotImplementedError

    def eval(self, contractor=None, dtype=None):
        ...

    def to_tn(self, dtype=None):
        ...

    def grad(self, var, **params):
        ...
\end{minted}

Each of the static methods of \py{tensor.Diagram} above comes with a
corresponding subclass of \py{Box}
with a special \py{__init__} method. For example the class \py{Spider} stores
a spider as a pair of \py{int} for the numbers of input and output legs and
a \py{dim:int} for the dimension of each leg.

\begin{minted}{python}
class Box(rigid.Box, Diagram):
        """ Box in a tensor.Diagram """
        def __init__(self, name, dom, cod, data, **params):
            rigid.Box.__init__(self, name, dom, cod, data=data, **params)
            Diagram.__init__(self, dom, cod, [self], [0])

        @property
        def array(self):
            """ The array inside the box. """
            dom, cod = self.dom, self.cod
            data = self.data
            try:
                return Tensor.np.array(data).reshape(tuple(dom @ cod) or ())
            except Exception:
                return data

        def grad(self, var, **params):
            return self.bubble(
                func=lambda x: getattr(x, "diff", lambda _: 0)(var),
                drawing_name="$\\partial {}$".format(var))

        def __repr__(self):
            return super().__repr__().replace("Box", "tensor.Box")

        def __eq__(self, other):
            if not isinstance(other, Box):
                return False
            return Tensor.np.all(Tensor.np.array(self.array == other.array))\
                and (self.name, self.dom, self.cod)\
                == (other.name, other.dom, other.cod)

class Id(rigid.Id, Diagram):
    """ Identity tensor.Diagram """
    def __init__(self, dom=Dim()):
        rigid.Id.__init__(self, dom)
        Diagram.__init__(self, dom, dom, [], [], layers=cat.Id(dom))

        class Swap(rigid.Swap, Diagram):
            """ Symmetry in a tensor.Diagram """


class Spider(rigid.Spider, Box):
    def __init__(self, n_legs_in, n_legs_out, dim):
        dim = dim if isinstance(dim, Dim) else Dim(dim)
        rigid.Spider.__init__(self, n_legs_in, n_legs_out, dim)
        array = numpy.zeros(self.dom @ self.cod)
        for i in range(int(numpy.prod(dim))):
            array[len(self.dom @ self.cod) * (i, )] = 1
        Box.__init__(self, self.name, self.dom, self.cod, array)
        self.dim = dim
\end{minted}
\end{python}

TensorNetwork encodes tensor networks as nodes with matchng
indices. It provides a special class \py{CopyNode} which corresponds to Frobenius
spiders. We can build an interface \py{to_tn} which scans through a \py{tensor.Diagram}
and constructs the corresponding TensorNetwork with copy nodes.

\begin{python}\label{listing:tensor.TensorNetwork}
{\normalfont Interface between \py{tensor.Diagram} and TensorNetwork.}

\begin{minted}{python}
import tensornetwork as tn

def to_tn(diagram, dtype):
    nodes = [
        tn.CopyNode(2, getattr(dim, 'dim', dim), f'input_{i}', dtype=dtype)
        for i, dim in enumerate(diagram.dom)]
    inputs, scan = [n[0] for n in nodes], [n[1] for n in nodes]
    for box, offset in zip(diagram.boxes, diagram.offsets):
        if isinstance(box, rigid.Swap):
            scan[offset], scan[offset + 1] = scan[offset + 1], scan[offset]
            continue
        if isinstance(box, Spider):
            dims = (len(box.dom), len(box.cod))
            if dims == (1, 1):  # identity
                continue
            elif dims == (2, 0):  # cup
                tn.connect(*scan[offset:offset + 2])
                del scan[offset:offset + 2]
                continue
            else:
                node = tn.CopyNode(sum(dims),
                                   scan[offset].dimension,
                                   dtype=dtype)
        else:
            array = box.eval().array
            node = tn.Node(array, str(box))
        for i, _ in enumerate(box.dom):
            tn.connect(scan[offset + i], node[i])
        scan[offset:offset + len(box.dom)] = node[len(box.dom):]
        nodes.append(node)
    return nodes, inputs + scan
\end{minted}
\end{python}

